MAVIS: A Benchmark for Multimodal Source Attribution in Long-form Visual Question Answering

Source attribution aims to enhance the reliability of AI-generated answers by including references for each statement, helping users validate the provided answers. However, existing work has primarily focused on text-only scenario and largely overlooked the role of multimodality. We introduce MAVIS, the first benchmark designed to evaluate multimodal source attribution systems that understand user intent behind visual questions, retrieve multimodal evidence, and generate long-form answers with citations. Our dataset comprises 157K visual QA instances, where each answer is annotated with fact-level citations referring to multimodal documents. We develop fine-grained automatic metrics along three dimensions of informativeness, groundedness, and fluency, and demonstrate their strong correlation with human judgments. Our key findings are threefold: (1) LVLMs with multimodal RAG generate more informative and fluent answers than unimodal RAG, but they exhibit weaker groundedness for image documents than for text documents, a gap amplified in multimodal settings. (2) Given the same multimodal documents, there is a trade-off between informativeness and groundedness across different prompting methods. (3) Our proposed method highlights mitigating contextual bias in interpreting image documents as a crucial direction for future research.

==> Tables/controlled_experiment.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{c||c|c}
\toprule
\#Txt & Img Grd. & Img Util.\\
\midrule
0 & &  \\
1 & &  \\
2 & &  \\
3 & &  \\
4 & &  \\
5 & &  \\
\bottomrule
\end{tabular}
\caption{.}
\vspace{-2mm}
\label{tab:corr_human}
\end{table}

==> Tables/gt_compare.tex <==
\definecolor{graycustom}{HTML}{2f2f2f}

\begin{table}[!t]
\centering
% \small
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{Informativeness} & \multicolumn{1}{c}{Groundedness} & Fluency\\
 \cmidrule(lr{2mm}){2-2}\cmidrule(lr{2mm}){3-3}\cmidrule(lr{2mm}){4-4}
 & \multicolumn{1}{c}{F1-score} & \multicolumn{1}{c}{F1-score} & \multicolumn{1}{c}{MAUVE} \\
\midrule
\rowcolor{gray!20}\multicolumn{4}{c}{\textbf{\text{Qwen2.5VL}}}\\
Text-RAG & 30.7 & 77.9 & \textbf{56.9} \\
Image-RAG & 30.7 & 49.2 & 38.7 \\
Multi-RAG & 32.3 & 72.0 & \underline{50.8} \\
GT Text-RAG & N/A & N/A & N/A \\
GT Image-RAG & \textul{36.1} & 50.1 & 32.2 \\
GT Multi-RAG & \textbf{42.4} & 55.5 & 44.2 \\

\rowcolor{gray!20}\multicolumn{4}{c}{\textbf{\text{GPT-4o}}}\\
Text-RAG & 37.0 & \textbf{73.4} & 69.7 \\
Image-RAG & 43.2 & 35.7 & 71.5 \\
Multi-RAG &  49.4 & 64.3 & \underline{73.3} \\
GT Text-RAG & 50.7 & \underline{65.0} & 71.1\\
GT Image-RAG & \underline{53.8} & 36.9 & \textbf{73.5} \\
GT Multi-RAG & \textbf{56.3} & 62.6 &  70.6 \\
\bottomrule

\end{tabular}
}

\caption{Performance of RAG using retrieved documents ($N=1$, $K=5$) and ground-truth documents. For the ground-truth setting, up to five documents are randomly selected from the ground-truth set.}

\label{table:gt_compare}
\vspace{-3mm}
\end{table}

